Shaping Frequency-Bin Biphoton Correlations via Programmable Optical Frequency Combs

Programmable shaping of photon-pair spectral correlations is important for frequency-bin quantum information processing. However, achieving this control remains challenging in nonlinear optical systems without reliable forward models. Here, we demonstrate model-free, hardware-in-the-loop shaping of the measured joint spectral intensity of a cascaded photon-pair source driven by a programmable optical frequency comb. A blockwise simultaneous perturbation stochastic approximation controller optimizes up to 22 pump, signal, and idler parameters. Each iteration requires only two accepted hardware evaluations, independent of the parameter count. The controller converges to diverse target patterns on 3$\times$3, 4$\times$4, and 5$\times$5 frequency-bin grids. The optimized distributions achieve Pearson correlations between 0.66 and 0.98 and classical overlap fidelities between 0.32 and 0.62. Cross-target similarity analysis confirms that the optimized patterns remain target-specific. Source characterization yields a maximum coincidence-to-accidental ratio of approximately 585. Accuracy is limited by pump-phase transfer, parasitic nonlinear background, waveshaper constraints, amplitude-only filtering, and measurement noise. Joint spectral intensity contains no spectral-phase information. Therefore, the results demonstrate control of measured frequency-bin populations and correlations, not complete reconstruction of the two-photon state. Phase-sensitive characterization is required to verify inter-bin coherence and quantify the entanglement dimensionality of the output state. Our results establish direct measurement feedback as a practical approach to reconfigurable frequency-bin correlation engineering when an accurate end-to-end model is unavailable.

==> images/diagram.tex <==
\definecolor{ambergold}{HTML}{FFBE0B}
\definecolor{blazeorange}{HTML}{FB5607}
\definecolor{neonpink}{HTML}{FF006E}
\definecolor{blueviolet}{HTML}{8338EC}
\definecolor{azureblue}{HTML}{3A86FF}

\begin{tikzpicture}[>=Stealth, line cap=round, line join=round, font=\sffamily]
 \begin{scope}[scale=0.9]
     

% ---------- reusable pics ----------
\tikzset{
  % perturbed-spectrum bar plot (heights passed via macro)
  barsA/.pic={
    \draw[->, line width=1pt, pic actions] (0,0) -- (2.35,0);
    \draw[->, line width=1pt, pic actions] (0,0) -- (0,1.05);
    \foreach \x/\h in {0.15/0.55, 0.5/0.85, 0.85/0.35, 1.25/0.70, 1.6/0.25, 1.95/0.75}
      \draw[pic actions, fill, fill opacity=0.25] (\x,0) rectangle ++(0.2,\h);
  },
  barsB/.pic={
    \draw[->, line width=1pt, pic actions] (0,0) -- (2.35,0);
    \draw[->, line width=1pt, pic actions] (0,0) -- (0,1.05);
    \foreach \x/\h in {0.15/0.30, 0.5/0.65, 0.85/0.80, 1.25/0.40, 1.6/0.70, 1.95/0.30}
      \draw[pic actions, fill, fill opacity=0.25] (\x,0) rectangle ++(0.2,\h);
  },
  % amplitude frequency comb
  comb/.pic={
    \draw[->, line width=1pt, pic actions] (0,0) -- (2.35,0);
    \draw[->, line width=1pt, pic actions] (0,0) -- (0,1.05);
    \foreach \x in {0.30,0.65,...,2.05}
      \draw[pic actions, line width=0.9pt]
        ({\x-0.11},0) .. controls ({\x-0.02},0.03) and ({\x-0.045},0.62) .. (\x,0.62)
                      .. controls ({\x+0.045},0.62) and ({\x+0.02},0.03) .. ({\x+0.11},0);
  },
  % anti-diagonal JSI lobes
  jsi/.pic={
    \draw[->, line width=1pt, pic actions] (0,0) -- (2.2,0) node[right, pic actions]{$\omega_i$};
    \draw[->, line width=1pt, pic actions] (0,0) -- (0,2.1) node[above, pic actions]{$\omega_s$};
    \foreach \cx/\cy in {0.95/1.75, 1.35/1.35, 1.75/0.95}
      \draw[pic actions, fill, fill opacity=0.22, rotate around={-45:(\cx,\cy)}]
        (\cx,\cy) ellipse [x radius=0.58, y radius=0.15];
    \draw[pic actions, fill, fill opacity=0.22, rotate around={-45:(0.62,1.10)}]
      (0.62,1.10) ellipse [x radius=0.17, y radius=0.09];
    \draw[pic actions, fill, fill opacity=0.22, rotate around={-45:(1.10,0.62)}]
      (1.10,0.62) ellipse [x radius=0.17, y radius=0.09];
  }
}
 
% ---------- soft pastel backdrop (no dark background) ----------
\begin{scope}[on background layer]
\shade[left color=neonpink!7, right color=azureblue!9, rounded corners=14pt]
  (-0.7,-3.5) rectangle (15.4,5.1);
\end{scope}
 
% ================= perturbed pump inputs (left) =================
\begin{scope}[shift={(0,-0.5)}]
  % back panel: theta-eps*Delta, offset down-right, own isolating square
  \begin{scope}[shift={(0,0)}]
    \draw[draw=blazeorange!55, line width=1pt, rounded corners=8pt,
          fill=blazeorange!8, fill opacity=0.5]
      (-0.10,-0.40) rectangle (3.15,3.15);
    \node[blazeorange, anchor=west, font=\sffamily\bfseries] at (0.30,2.95) {$\theta-\epsilon\Delta$};
    \pic[blazeorange, fill opacity=0.96] at (0.35,1.45) {barsB};
    \node[ambergold!60!blazeorange, font=\sffamily\bfseries] at (0.12,1.02) {$A$};
    \pic[ambergold!75!blazeorange, opacity=0.7] at (0.35,0.00) {comb};
  \end{scope}
  % front panel: theta+eps*Delta, own isolating square
  \begin{scope}[shift={(0.35,-0.35)}]
  \draw[draw=blueviolet!55, line width=1pt, rounded corners=8pt,
        fill=azureblue!8, fill opacity=0.85]
    (-0.10,-0.40) rectangle (3.15,3.15);
  \node[blueviolet, anchor=west, font=\sffamily\bfseries] at (0.30,2.95) {$\theta+\epsilon\Delta$};
  \pic[blueviolet, fill opacity=0.7] at (0.35,1.45) {barsA};
  \node[azureblue, font=\sffamily\bfseries] at (0.12,1.02) {$A$};
  \pic[azureblue, opacity=0.95] at (0.35,0.00) {comb};
  \end{scope}
\end{scope}

% ================= SHG -> SPDC chain =================
\node[draw=blueviolet, line width=1.6pt, rounded corners=3pt,
      top color=neonpink!18, bottom color=blueviolet!18,
      minimum width=1.8cm, minimum height=1.0cm,
      font=\sffamily\bfseries\large, text=blueviolet] (shg) at (5.95,0.85) {S\,H\,G};
 
\node[draw=neonpink, line width=1.6pt, rounded corners=3pt,
      top color=azureblue!16, bottom color=neonpink!16,
      minimum width=1.8cm, minimum height=1.0cm,
      font=\sffamily\bfseries\large, text=neonpink] (spdc) at (8.75,0.85) {S\,P\,D\,C};
 
% narrow feed arrows into SHG (keep them thin)
\draw[->, blazeorange!70, line width=0.55pt] (2.95,2.64) to[out=0,in=-180] ($(shg.west)+(0,0.22)$);
\draw[->, blazeorange!70, line width=0.55pt] (3.53,-0.52) to[out=50,in=-180] ($(shg.west)+(0,0.07)$);
\draw[->, blueviolet!65, line width=0.55pt] (3.25,2.3) to[out=0,in=180] ($(shg.west)+(0,-0.07)$);
\draw[->, blueviolet!65, line width=0.55pt] (3.25,-1.25) to[out=0,in=180] ($(shg.west)+(0,-0.22)$);

 
% SHG -> SPDC arrow with the slash
\draw[->, line width=1.4pt, blueviolet] (shg.east) -- (spdc.west);
\path (shg.east) -- (spdc.west) coordinate[midway] (mid);
\draw[neonpink, line width=1.3pt] ($(mid)+(-0.13,-0.20)$) -- ($(mid)+(0.13,0.20)$);
 
% ================= JSI panels (right, no output arrows) =================
\begin{scope}[shift={(10.85,-0.35)}]
  % back layer: JSI- , slightly offset down-right, own isolating square
  \begin{scope}[shift={(0,0)}]
    \draw[draw=neonpink!55, line width=1pt, rounded corners=10pt,
          fill=neonpink!8, fill opacity=0.5]
      (-0.55,-0.55) rectangle (3.05,2.85);
    \pic[neonpink, fill opacity=0.6] at (0,0) {jsi};
    \node[neonpink,   font=\sffamily\bfseries] at (1.65,2.65) {JSI$^{\,-}$};
  \end{scope}
  % front layer: JSI+ , at nominal position, own isolating square
  \begin{scope}[shift={(0.4,-0.4)}]
      \draw[draw=blueviolet!55, line width=1pt, rounded corners=10pt,
            fill=azureblue!8, fill opacity=0.93]
        (-0.55,-0.55) rectangle (3.05,2.85);
      \pic[azureblue, fill opacity=0.8] at (0,0) {jsi}; 
      \node[blueviolet, font=\sffamily\bfseries] at (1.65,2.65) {JSI$^{\,+}$};
  \end{scope}
  
\end{scope}
  \end{scope}
\end{tikzpicture}

==> images/representatives/representatives.tex <==


\begin{tikzpicture}[font=\sffamily\small, every node/.style={align=center}, circuitikz/bipoles/length=0.6cm]

\tikzset{
  fiber/.style={
    draw=yellow!80!black,
    line width=1.5pt,
    line cap=round,
    line join=round,
    shorten <= 0.4pt,
    shorten >= 0.4pt
  }
}
\tikzset{
  free_space_directed/.style={
    draw=red,
    line width=1.5pt,
    line cap=round,
    line join=round,
    shorten <= 0.4pt,
    shorten >= 0.4pt,
    ->, 
    >=stealth % Makes the arrowhead look sleek and standard
  }
}

% TLS image node
\node (3p) [inner sep=0pt, outer sep=0pt, anchor=center]
  {\includegraphics[width=7.4cm]{images/representatives/representatives_3x3.pdf}};
\node (a) at ($(3p.west)+(0.4,3)$) {(a)};

\node (4p) at ($(3p.east)+(3.75,0)$) {\includegraphics[width=7.4cm]{images/representatives/representatives_4x4.pdf}};
\node (b) at ($(4p.west)+(0.4,3)$) {(b)};

\node (4p2) at ($(3p.south)+(0,-3)$) {\includegraphics[width=7.4cm]{images/representatives/representatives_4x4_2.pdf}};
\node (c) at ($(4p2.west)+(0.4,3)$) {(c)};

\node (5p) at ($(4p2.east)+(3.75,0)$){\includegraphics[width=7.4cm]{images/representatives/representatives_5x5.pdf}};
\node (d) at ($(5p.west)+(0.4,3)$) {(d)};

\end{tikzpicture}

==> images/results/similarity.tex <==
\begin{tikzpicture}[font=\sffamily\tiny, every node/.style={align=center}, circuitikz/bipoles/length=0.6cm]

\tikzset{
  fiber/.style={
    draw=yellow!80!black,
    line width=1.5pt,
    line cap=round,
    line join=round,
    shorten <= 0.4pt,
    shorten >= 0.4pt
  }
}
\tikzset{
  free_space_directed/.style={
    draw=red,
    line width=1.5pt,
    line cap=round,
    line join=round,
    shorten <= 0.4pt,
    shorten >= 0.4pt,
    ->, 
    >=stealth % Makes the arrowhead look sleek and standard
  }
}

% TLS image node
\node (3p) [inner sep=0pt, outer sep=0pt, anchor=center]
  {\includegraphics[width=6.5cm]{images/results/png_similarity_matrix_3mp.pdf}};
\node (4p) at ($(3p.east)+(2.5,0)$) {\includegraphics[width=6.5cm]{images/results/png_similarity_matrix_4mp.pdf}};

\node (5p) at ($(4p.east)+(2.5,0)$) {\includegraphics[width=6.5cm]{images/results/png_similarity_matrix_5mp.pdf}};

\end{tikzpicture}

==> images/setup/mQPG.tex <==
\begin{tikzpicture}[font=\small, line cap=round, line join=round]

    % Define colors
    \definecolor{myPurple}{RGB}{180, 120, 255}

    % Optional: Grid to match your reference image
    \draw[help lines, thin, dotted, step=0.05] (0,-0.1) grid (0.6,0.1);

    % The Path
    \draw[myPurple, thick] 
        (0,0) -- (0.6,0)                           % Initial flat line
        .. controls (0.8,0) and (0.6,0.2) .. (0.8,0.2) % The S-curve (Bézier)
        -- (0.9,0.2);                                % Final flat line

    \draw[] 
        (0,-0.1) -- (0.9,-0.1) -- (0.9,0.3) -- (0,0.3) -- (0,-0.1); 
    % The Label (matching the "7wp" in the image)
    %\node[myPurple, font=\ttfamily\bfseries] at (5.7,0.5) {7wp};

\end{tikzpicture}


==> images/setup/spectrograph.tex <==
\usetikzlibrary{circuits.logic.US, positioning}

\begin{tikzpicture}[font=\sffamily\scriptsize, every node/.style={align=center}, circuitikz/bipoles/length=1cm]
  % Two colored outputs from the right side of the waveguide
\draw[thick, green!70!black] (-1.5,0.1) -- (-1.25,0.1);
\draw[thick, orange!90!black] (-1.5,0) -- (-1.25,0);
\draw[thick, red!90!black] (-1.5,-0.1) -- (-1.25,-0.1);

  % Half-circle with flat right side
  \draw (-1,0.25) arc[start angle=-270, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node at (-1,0.75) {Coupler};
  \node at (-2.5,0) {\textbf{mQPG} \\ \textbf{WG}};

  \draw[draw=red, line width=2pt] (-1,0) -- (1.2,0);

  % Diagonal outputs (e.g., LEDs)
  \foreach \i in {0,...,5} {
    \draw (1,0.3) -- ++(\i*0.1,-\i*0.125);
    \filldraw (1,0.3) ++(\i*0.1,-\i*0.125) circle (0.05);
  }
 \node[align=center] at (1.2,1) {Diffraction \\ grating};

  % Vertical lines (each with a label)
  \draw (-1,-1) -- (-1,-2);
  \node at (-1.4,-1.5) {$m_1$};

  \draw (1.2,-2) -- (1.2,-3);
  \node at (1.6,-2.5) {$m_2$};

  \draw (-1,-3) -- (-1,-4);
  \node at (-1.4,-3.5) {$m_3$};

  \draw (1.2,-4) -- (1.2,-5);
  \node at (1.6,-4.5) {$m_4$};

  \draw (-1,-5) -- (-1,-6);
  \node at (-1.4,-6.5) {$m_5$};

  \draw (1.2,-6) -- (1.2,-7);
  \node at (1.6,-7.5) {$m_6$};

  \draw (-1,-7) -- (-1,-7.5);
  \node at (-1.4,-7.75) {$m_7$};

  \draw (-1,-8) -- (-1,-8.5);
  \node at (-1.4,-8.75) {$m_8$};

  \draw (-1,-9) -- (-1,-9.5);
  \node at (-1.4,-9.75) {$m_9$};

  % Green path
  \draw[green!70!black, line width=1.5pt] (1.2,0) -- (-1,-1.4) -- (1.2,-2.3) -- (-1,-3.2) -- (1.2,-4.1) -- (-1,-5.25) -- (1.7,-6.1);

  % Orange path
  \draw[draw=orange!90!black, line width=1.5pt] (1.2,0) -- (-1,-1.5) -- (1.2,-2.45) -- (-1,-3.5) -- (1.2,-4.6) -- (-1,-6.25) -- (1.7,-7.1);

  % Blue path
  \draw[draw=red!90!black, line width=1.5pt] (1.2,0) -- (-1,-1.6) -- (1.2,-2.7) -- (-1,-3.8) -- (1.2,-5) -- (-1,-7.25) -- (1.7,-8.1);

  %% Photodetectors
  \draw (1.7,-5.8) arc[start angle=90, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node (c1) at (1.8,-6.1) {};
  \node (spd1) [right=0.2cm of c1, draw, rectangle, minimum width=1cm, minimum height=0.5cm] {SPD$_1$};
  \draw (c1.east)--(spd1.west);
  \draw[draw=green!40!black, line width=1.5pt] (0.9,-5.6) -- (0.8,-6.1);  \draw[draw=green!40!black, line width=1.5pt] (1.1,-5.7) -- (1.0,-6.2);
  \node at (1.2,-6.2) {$f_1$};

  \draw (1.7,-6.8) arc[start angle=90, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node (c2) at (1.8,-7.1) {};
  \node (spd2) [right=0.2cm of c2, draw, rectangle, minimum width=1cm, minimum height=0.5cm] {SPD$_2$};
  \draw (c2.east)--(spd2.west);
  \draw[draw=orange!40!black, line width=1.5pt] (0.9,-6.6) -- (0.8,-7.1);
  \node at (1,-7) {};
  \draw[draw=orange!40!black, line width=1.5pt] (1.1,-6.7) -- (1.0,-7.2);
  \node at (1.2,-7.2) {$f_2$};
  
  \draw (1.7,-7.8) arc[start angle=90, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node (c3) at (1.8,-8.1) {};
  \node (spd3) [right=0.2cm of c3, draw, rectangle, minimum width=1cm, minimum height=0.5cm] {SPD$_3$};
  \draw (c3.east)--(spd3.west);
  \draw[draw=red!40!black, line width=1.5pt] (0.9,-7.6) -- (0.8,-8.1);
  \node at (1,-8) {};
  \draw[draw=red!40!black, line width=1.5pt] (1.1,-7.7) -- (1.0,-8.2);
  \node at (1.2,-8.2) {$f_3$};

  
  \node (pc) at (4.5,-7.1){\includegraphics[width=1.25cm]{images/setup/PC.png}};
  \node at ($(pc.south)+(0,-0.1)$) {PC};

  \draw (spd1.east) -- (pc.west);
  \draw (spd2.east) -- (pc.west);
  \draw (spd3.east) -- (pc.west);
\end{tikzpicture}

